CURing Large Models: Compression via CUR Decomposition

Large deep learning models have achieved remarkable success but are resource-intensive, posing challenges such as memory usage. We introduce CURing, a novel model compression method based on CUR matrix decomposition, which approximates weight matrices as the product of selected columns (C) and rows (R), and a small linking matrix (U). We apply this decomposition to weights chosen based on the combined influence of their magnitudes and activations. By identifying and retaining informative rows and columns, CURing significantly reduces model size with minimal performance loss. For example, it reduces Llama3.1-8B's parameters to 7.32B (-9%) in just 129 seconds, over 20 times faster than prior compression methods.

==> texts/2_img_curlora.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.32\textwidth]{images/curlora.png}
    \caption{
        Visualization of the
        \textbf{Compression + CURLoRA}.
    }
    \label{fig:curlora}
\end{figure}


==> texts/5_3_1_heal_table.tex <==
\begin{table*}[!th]
\footnotesize
\centering
\caption{Comparison of Frobenius Norm values and differences across layers (\textit{Frobenius Norm} above, \textit{difference} between teacher and student (\(\| W - CUR \|_F\)) below in parentheses; layers are sorted by angular distance difference in ascending order).}  % TODO: N10, (Llama3.1-8B)
\resizebox{\textwidth}{!}{%
\begin{tabular}{c*{10}{|r}}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{10}{c}{\textbf{Layers Sorted by Angular Distance}} \\ \cline{2-11}
                & \multicolumn{1}{c|}{\textbf{25}}   & \multicolumn{1}{c|}{\textbf{26}}   & \multicolumn{1}{c|}{\textbf{27}}   & \multicolumn{1}{c|}{\textbf{24}}   & \multicolumn{1}{c|}{\textbf{28}}  & \multicolumn{1}{c|}{\textbf{23}}  & \multicolumn{1}{c|}{\textbf{22}}  & \multicolumn{1}{c|}{\textbf{29}}  & \multicolumn{1}{c|}{\textbf{20}}  & \multicolumn{1}{c}{\textbf{21}}  \\ \hline \hline
\multirow{1}{*}{Teacher} 
                & 210.28 & 212.11 & 214.05 & 209.34 & 215.03 & 208.87 & 207.97 & 217.90 & 207.28 & 208.14 \\ \hline \hline
\multirow{2}{*}{Student} 
                & 156.10 & 157.74 & 160.65 & 154.93 & 162.56 & 153.10 & 152.28 & 166.21 & 150.76 & 151.75 \\ 
                & (140.90) & (141.81) & (141.45) & (140.78) & (140.76) & (142.09) & (141.65) & (140.90) & (142.25) & (142.47) \\ \hline
\multirow{2}{*}{\shortstack{Student\\(Healed)}}
                & 330.00 & 340.00 & 350.00 & 360.00 & 370.00 & 380.00 & 390.00 & 400.00 & 410.00 & 420.00 \\ 
                & (-1990.00) & (+2030.00) & (-2070.00) & (+2110.00) & (-2150.00) & (+2190.00) & (-2230.00) & (+2270.00) & (-2310.00) & (+2350.00) \\ \hline
\end{tabular}%
}
\end{table*}

==> texts/6_2_future_work.tex <==
% \subsection{Future Research Directions}


% While CURing demonstrates effectiveness in compressing models, several avenues exist for further exploration.


% \paragraph{Optimal Rank Selection}
% %
% Selecting an appropriate rank \( r \) is crucial for balancing compression and performance.
% Future work could focus on exploring more advanced methods for rank selection, potentially employing layer-specific ranks based on their relative influence (angular distance).


% \paragraph{Advanced Decomposition Methods}
% %
% Exploring alternative decomposition techniques could yield more efficient or compact representations.
% %
% For instance, the Compact Matrix Decomposition (CMD) or other approaches proposed in prior research~\cite{sun2007less,ekenta2022spectrum} offer smaller and faster decomposition ways for sparse matrices.


==> texts/E_1_heatmap.tex <==
% https://tex.stackexchange.com/questions/133882/create-heatmap-with-pstricks-or-tikz

% TODO:
% Healing/C128_N10 기준. 기본값.
% 마지막 레이어 q, k, gate 히트맵 보면 될 듯. 수치도 같이 저장하자.


==> texts/G_1_sparsity_table.tex <==
\begin{table*}[!th]
\footnotesize
\centering
\caption{Comparison of the sparsity between original model (Llama3.1-8B) and the CURing-applied model.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c*{16}{|r}}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{16}{c}{\textbf{Number of Compressed Layers}} \\ \cline{2-17}
                & \multicolumn{1}{c|}{\textbf{0}}   & \multicolumn{1}{c|}{\textbf{2}}   & \multicolumn{1}{c|}{\textbf{4}}   & \multicolumn{1}{c|}{\textbf{6}}   & \multicolumn{1}{c|}{\textbf{8}}  & \multicolumn{1}{c|}{\textbf{10}}  & \multicolumn{1}{c|}{\textbf{12}}  & \multicolumn{1}{c|}{\textbf{14}}  & \multicolumn{1}{c|}{\textbf{16}}  & \multicolumn{1}{c|}{\textbf{18}}  & \multicolumn{1}{c|}{\textbf{20}}  & \multicolumn{1}{c|}{\textbf{22}}  & \multicolumn{1}{c|}{\textbf{24}}  & \multicolumn{1}{c|}{\textbf{26}}  & \multicolumn{1}{c|}{\textbf{28}}  & \multicolumn{1}{c}{\textbf{30}}  \\ \hline \hline
\multirow{1}{*}{Original} 
                & 99.14 & 89.93 & 24.87 & 75.72 & 6.24 & 52.31 & 88.99 & 31.45 & 67.11 & 29.52 & 78.68 & 21.36 & 44.69 & 16.22 & 93.11 & 59.88 \\ \hline
\multirow{1}{*}{CURing} 
                & 69.57 & 67.33 & 44.01 & 38.41 & 81.51 & 22.47 & 54.36 & 77.82 & 18.34 & 40.61 & 63.29 & 92.55 & 28.71 & 50.39 & 11.23 & 33.87 \\ \hline
\end{tabular}%
}
\end{table*}

==> texts/G_sparsity.tex <==
\section{Sparsity} \label{appendix:sparsity}

\input{texts/G_1_sparsity_table}

\textcolor{red}{WIP}

